A Far-ultraviolet Atlas of Low-resolution Hubble Space Telescope Spectra of T Tauri Stars

We present a far-ultraviolet (FUV) spectral atlas consisting of spectra of 91 pre-main sequence stars. Most stars in this sample were observed with the Space Telescope Imaging Spectrograph (STIS) and Advanced Camera for Surveys (ACS) on the \emph{Hubble Space Telescope} (\emph{HST}). We find strong correlations among the \ion{O}{1} $\lambda$1304 triplet, %\ion{C}{2} $\lambda$1335, the \ion{Si}{4} $\lambda\lambda$1394/1403 doublet, the \ion{C}{4} $\lambda$1549 doublet, and the \ion{He}{2} $\lambda$1640 line luminosities. For classical T Tauri stars (CTTSs), we also find strong correlations between these lines and the accretion luminosity, suggesting that these lines form in processes related to accretion. These FUV line fluxes and X-ray luminosity correlate loosely with large scatters. The FUV emission also correlates well with H$\alpha$, H$\beta$, and \ion{Ca}{2} K line luminosities. These correlations between FUV and optical diagostics can be used to obtain rough estimates of FUV line fluxes from optical observations. Molecular hydrogen (H$_{2}$) emission is generally present in the spectra of actively accreting CTTSs but not the weak-lined T Tauri stars (WTTSs) that are not accreting. The presence of H$_2$ emission in the spectrum of HD 98800 N suggests that the disk should be classified as actively accreting rather than a debris disk. The spectra in the atlas are available at http://archive.stsci.edu/prepds/ttauriatlas.

==> table2_2011aug9.tex <==

%Target properties
%new table, Sept. 2
\begin{deluxetable}{llccccrrrrrrc}
\rotate
 \tablewidth{0pt}
 \tablecaption{ Pre-Main Sequence Stars. \label{pmstable}}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{ID} &\colhead{Name}&\colhead{Region} %&\colhead{Type}%&\colhead{Category}
&\colhead{Distance (pc)} & \colhead{Type\tablenotemark{a}} & \colhead{Category}  &\colhead{$A_{V}$}
&\colhead{log$L_{phot}$\tablenotemark{b}}& \colhead{log$L_{acc}$\tablenotemark{c}}  
& \colhead{log$L_{\rm{X}}$\tablenotemark{d}}&\colhead{H$\beta$\tablenotemark{e}} &\colhead{Ca II K\tablenotemark{e}}
&\colhead{Reference \tablenotemark{f}}
}
\startdata                                % d                Av   Lphot  Lacc    Lx     Hbeta  CaII K  Ref
                                     %                                                10^-14   10^-14
1 &DK Cet                  &   field       & 42& G4    &WTTS& 0.0& -0.05&...   &...   &  ...  & ...  & 1,2 \\ 
2 &\Lkha 330               &   Per        &250& G3    &CTTS& 1.8&  1.2 &...   &...   &  ...  & ...  &  3 \\
3 &2M0414                  &   Taurus     &140& M6.25 &CTTS& 0.7& -1.90& -2.50&...   &  2.50 & 1.90 & 4 \\ 
4 &FM Tau                  &   Taurus     &140& M1    &CTTS& 0.3  & -0.77& -1.7 & 29.7 &  17.8 & 3.32 &5 \\
5 &FP Tau                  &   Taurus     &140& M4    &CTTS& 0.0  & -0.57 & -2.8  &...   &  10.7 & 1.54 &  5 \\
6 &CX Tau                  &   Taurus     &140& M2.5  &CTTS& 0.2 & -0.48 & -2.6 &...   &  14.9 & 2.12 &5 \\
7 &LkCa 3                  &   Taurus     &140& M1    &WTTS& 0.4 &   0.04& ...   &...   &  2.42 & 4.35 &         6 \\ 
8 &LkCa 4                  &   Taurus     &140& K7    &WTTS& 1.2&  -0.02 &...   &...   &  5.86 & 4.30 &      5 \\ 
9 &CY Tau                  &   Taurus     &140& M2    &CTTS& 0.3& -0.34& -1.39&      &  54.8 & 8.89 & 7 \\
10&BP Tau                  &   Taurus     &140& K7    &CTTS& 0.5& -0.03& -0.75&      &  85.5 & 20.5 & 7 \\
11&LkCa 7                  &   Taurus     &140&M0+M3.5&WTTS& 0.6 &  -0.14  &...   &...   &  5.40 & 3.65 &        6 \\ 
12&DE Tau                  &   Taurus     &140& M2    &CTTS& 0.6& -0.06& -1.15&...   &  6.58 & 5.68 & 7 \\ 
13&RY Tau                  &   Taurus     &140& F8    &CTTS& 1.8   &  0.89  &   ...   & 30.7 &  ...  & ...  &    8\\ 
14&T Tau                   &   Taurus     &140& K0    &CTTS& 1.5 &  0.86  &  -0.29 & 31.0 &  517 & 261 &  5 \\ 
15&IP Tau                  &   Taurus     &140& M0    &CTTS& 0.3 & -0.39& -2.15&...   &  14.7 & 4.26 & 7 \\ 
16&DF Tau                  &   Taurus     &140& M2    &CTTS& 0.6&  0.16& -0.75&...   &  1567 & 31.7 & 4 \\
17&HBC 388                 &   Taurus     &140& K1    &WTTS?& 0.0 &  0.13&...   &...   &  ...  & ...  &          5 \\
18&V827 Tau                &   Taurus     &140& K7    &WTTS& 1.1&  0.04  &...   & 30.6 &  6.22 & 5.02 & 5 \\ 
19&V826 Tau                &   Taurus     &140& K7    &WTTS& 0.3&   -0.10       &...   & 30.6 &  6.09 & 4.31 &6\\ 
20& MHO 6                  &   Taurus     &140& M5    &CTTS& 1.0 & -0.85& -2.80&...   &  1.60 & 0.45 & 4 \\
21&UZ Tau W                &   Taurus     &140&M1+M4  &CTTS& 1.0 & -0.20& -1.5 &...   &  16.5 & 2.86 & 5\\
22&UZ Tau E                &   Taurus     &140&M2+M3  &CTTS& 0.3& -0.51& -1.6  &...   &  34.8 & 33.6      & 5\\
23&V830 Tau                &   Taurus     &140& K7    &WTTS& 0.7& -1.01&...   & 30.7 &  4.08 & 4.63 &  5 \\ 
24&GI Tau                  &   Taurus     &140& K7    &CTTS& 1.3& -0.07& -1.03&...   &  3.11 & 0.74 & 7\\
25&GK Tau                  &   Taurus     &140& K7    &CTTS& 0.9&  0.03& -1.46& 30.1 &  11.1 & 4.14 & 7 \\
26&DL Tau                  &   Taurus     &140& K7    &CTTS& 1.3& ...  & -0.65  &...   &  60.9 & 38.1       & 9 \\
27&HN Tau A                &   Taurus     &140& K5    &CTTS& 0.6 & -0.72& -1.45& 29.2 &  28.8 & 38.9 & 7 \\
28&HN Tau B                &   Taurus     &140& M4.5  &CTTS&0.9 & -1.60& ...  &...   &  2.47 & 1.84 &  5 \\
29&DM Tau                  &   Taurus     &140& M1    &CTTS& 0.6 & -0.61 & -1.5 & 29.3 &  24.1 & 2.98 &  5 \\
30&CI Tau                  &   Taurus     &140& K7    &CTTS& 1.8& -0.08&   -0.57   &...   &  44.4 & 29.4 & 5 \\
31&AA Tau                  &   Taurus     &140& K7    &CTTS&0.74& -0.13& -1.60&...   &  10.4 & 3.67 &  7\\
32&DN Tau                  &   Taurus     &140& M0    &CTTS& 1.9& -0.06& -1.79& 30.0 &  10.5 & 5.01 & 7 \\
33&DO Tau                  &   Taurus     &140& M0    &CTTS& 2.3&  0.00& -0.20&...   &  48.2 & 42.1 & 7 \\
34&2M0439                  &   Taurus     &140& M5    &CTTS& 0.0& -1.05& -3.20&...   &  1.54 & 0.59 & 4 \\
35&LkCa 15              &   Taurus     &140& K5    &CTTS& 1.0& -0.13 &  -1.6 &...   &  ...  & 6.64 & 5 \\
36&DP Tau                  &   Taurus     &140& M0.5  &CTTS& 1.2&  ...  & -1.4 &...   &  ...  & ...  & 9 \\
37&2M0444                  &   Taurus     &140& M7.25 &CTTS& 0.0& -1.92& -4.60&...   &  0.34 & 0.053& 7 \\
38&DR Tau                  &   Taurus     &140& K7    &CTTS& 1.2&  ... & -0.13&...   &  71.4 & 119  & 10 \\
39&DS Tau                  &   Taurus     &140& K5    &CTTS& 0.3& -0.24& -0.70&...   &  47.1 & 13.7 & 7\\
40&GM Aur                  &   Taurus     &140& K5    &CTTS& 0.3& -0.13& -1.15&      &  66.4 & 10.2 & 7 \\
41&SU Aur                  &   Taurus     &140& G2    &CTTS& 0.9&  0.89& -1.00& 31.1 &  ...  & ...  & 11 \\
42&V397 Aur                &   Taurus     &140& K5    &WTTS& 0.0&  -0.10   &...   & 30.5 &  ...  & 3.89 & 6 \\ %HBC 427
43&V836 Tau                &   Taurus     &140& K7    &CTTS& 1.1& -0.49& -2.50&...   &  9.44 & 1.46 &4\\
44&RW Aur AB               &   Taurus     &140& K4    &CTTS& 1.2 &...   &  0.64 &...   &  126  & 521  & 9 \\
45&2M0518                  &   Taurus     &140& M5    &CTTS& 1.0& 0.016& -2.55&...   &  1.51 & 0.43 &4 \\
46&CO Ori                  &$\lambda$ Ori &450& G0    &CTTS& 2.0&  1.35&  0.22&...   &  ...  & ...  &11\\
47&GW Ori                  &$\lambda$ Ori &450& G0    &CTTS& 1.3&  1.79&  0.67&...   &  ...  & ...  &11 \\
48&V1044 Ori               &  Ori OB 1c   &440& G2    &CTTS& 2.0&  0.83& -0.22&...   &  ...  & ...  &11 \\
49&EZ Ori                     &  Ori OB 1c   &440& G3    &CTTS& 0.6&  0.77& -1.00&...   &  ...  & ...  &11 \\
50&CQ Tau                    &             &130 & F2   &CTTS& 1.9&  0.82&...   &...   &  ...  & ...  &  12\\
51&Parenago 2441         &  Ori OB 1c   &440& F9    &CTTS& 0.4&  1.06& -0.40&...   &  ...  & ...  & 11  \\
52&HD 53143                &   field        &18.4&G8    &WTTS& 0.0&-0.30 &...   &...   &  ...  & ...  &  2,13 \\
53&HD 61005                &   field        & 35& G4    &WTTS& 0.0&-0.25 &...   &...   &  ...  & ...  &  2,1\\
54&TWA 6                     &   TWA        & 51& K7    &WTTS& 0.0&-0.93 &...   &...   &  19.9 & 9.71 & 14,15\\
55&TWA 7                   &   TWA        & 27& M1    &WTTS& 0.0&-1.09 &...   &...   &  29.8 & 22.9 & 14,15\\
56&V419 Hya                &   field      & 22& K0    &WTTS& 0.0& -0.43&...   &...   &  ...  & ...  &  2,16\\
57&TW Hya                  &   TWA        & 56& K7    &CTTS& 0.0& -0.77& -1.50&...   &  462  & 65.0 & 2,4\\
58&TWA 3 S                  &   TWA        & 34&M3.5   &WTTS& 0.0& -1.27&  ...  &...   &  6.92 & 6.46 & 14,17 \\
59&TWA 3 N                  &   TWA        & 34& M3    &CTTS& 0.0& -1.10& -2.50&...   &  47.9 & 12.3 & 14,17 \\
60&2M1111                  &   Cha I      &175& K1    &CTTS& 1.3& 0.33 &...   & 30.6 &  ...  & ...  & p07\\
61&TWA 13 N                 &   TWA        & 53& M1    &WTTS& 0.0&-0.77 &...   &...   &  20.2 & 14.7 &14,18\\
62&TWA 13 S                 &   TWA         & 53& M2    &WTTS& 0.0&-0.79 &...   &...   &  39.2 & 2.54 &14,18\\
63&HD 98800 N               &   TWA        & 40& K5(SB)&WTTS& 0.0&-0.38 &...   &...   &  ...  & ...  & 14,15\\
64&HD 98800 S               &   TWA        & 40& K5(SB)&WTTS& 0.0&-0.35 &...   &...   &  ...  & ...  & 14,15\\
65&TWA 8 S                  &   TWA        & 39& M5  &WTTS& 0.0&-1.66 &...   &...   &  2.65 & 1.47 & 14,15\\
66&TWA 8 N                  &   TWA        & 38& M2    &WTTS& 0.0&-1.04 &...   &...   &  22.5 & 14.8 &14,15\\
67&TWA 9 N                  &   TWA        & 56& M1  &WTTS& 0.0& -0.82 &...   &...   &  3.09 & 2.10 & 14,15\\
68&TWA 9 S                  &   TWA        & 69& K5    &WTTS& 0.0& -0.52 &...   &...   &  18.8 & 8.74 & 14,15\\
69&TWA 27                  &   TWA        &52.4&M8.25 &BD  & 0.0& -2.72& -5.30&...   &  0.341& 0.0128& 19,17 \\
70&TWA 16 N                 &   TWA        & 72& M1.5 &WTTS& 0.0&-0.74 &...   &...   &  ...  & ...  & 14,20\\
71&TWA 16 S                 &   TWA        & \multicolumn{6}{c}{Included in primary component}\\
72&MML 28                  &   field      &108& K2    &WTTS& 0.6&-0.37 &...   & 30.0 &  ...  & ...  & 21 \\
73&MML 34                  &  isolated?    & 86& K1    &CTTS& 1.2& 0.10 &...   & 30.2  &  ...  & ...  &  2\\
74&MML 36                  &   field      & 81& K0    &WTTS&0.0 & 0.0  &...   & 30.4 &  ...  & ...  & 21 \\
75&RU Lup                  &   Lup        &140& K7    &CTTS& 0.1& -0.22& -0.50&...   &  361  & 492  & 22\\
76&V1146 Sco               &   USco       &145& M0(B) &WTTS&0.0 & -0.41&...   &...   &  ...  & 1.27 & 23,24,25\\
77&HD 143006               &   USco       &145& G6    &CTTS& 1.6&  0.39&...   & 30.1  &  ...  & ...  & 23,26\\
78&RY Lup                  &   Lup        &140& K4    &CTTS&0.65&  0.42&...   &...   &  ...  & ...  &  27\\
79&V1154 Sco               &   USco       &145& K5(B) &WTTS& 0.4&  0.08&...   &...   &  ...  & ...  &  23,24,25\\
80&HO Lup                  &   Lup        &140& M1    &CTTS& 1.3&  0.30&...   &...   &  ...  & ...  & 28\\
81&V1157 Sco               &   USco       &145& K5    &WTTS& 1.0& -0.14&...   &...   &  ...  & 0.756& 23,24,25\\
82&V866 Sco                &   Oph       &125& K0    &CTTS& 2.2&  ...  & 0.16   &...   &  171  & 132  & 29,9\\
83&2M1614N                 &   USco       &145& K0    &CTTS & 1.5& 0.50&...   & 30.5 &  ...  & ...  & 23,26\\
84&2M1614S                 &   USco       &\multicolumn{6}{c}{Included in primary component}\\
85&V2129 Oph               &   Oph      &125& K6    &CTTS& 0.6&  0.23&...   &...   &  56.0 & 22.3 & 29,30,\\
86&V1121 Oph               &   Oph       &125& K5    &CTTS& 1.2&  redo & -0.6  &...   &  ...  & ...  &  29,31,9\\
87&V4046 Sgr               &  isolated    & 83& K5(SB)&CTTS& 0.0& -0.09&...   &...   &  ...  & ...  & \\
88&2M1842                  &   CrA       &130& K2    &CTTS& 1.0&  0.12&...   & 30.3 &  33.0 & 17.0 & 1,26,32\\
89&2M1852                  &   CrA       &130& K3    &CTTS& 0.9& -0.24&...   & 30.5 &  22.9 & 9.49 &1,26,32\\
90&AU Mic                  &      $\beta$ Pic    &9.9& M1    &WTTS&  -0.9  &    ...  & 29.5   &      &       &       &  20  \\
91&HD 202917               &   TucHor     & 46& G7    &WTTS& 0.0&-0.18 &...   &...   &  ...  & ...  &  16\\
%90&HD 202917               &   TucHor     & 46& G7    &WTTS& 0.0&-0.18 &...   &...   &  ...  & ...  &  p95,val05\\
\enddata
\tablenotetext{a}{``SB'' stands for spectroscopic binary and ``B'' stands for binary.}
\tablenotetext{b}{Photospheric luminosity is in units of solar luminosity.}
\tablenotetext{c}{Accretion luminosity in units of solar luminosity.}
\tablenotetext{d}{X-ray luminosity is in units of erg~$\rm{s^{-1}}$.}
\tablenotetext{e}{The fluxes of the H$\beta$ and \ion{Ca}{2} K lines are in units of $10^{-14}$ erg~$\rm{s^{-1}cm^{-2}}$.}
\tablenotetext{f}{References:  1:  \citet{White2007};  2:  \citet{Perryman1997}; 3:  \citet{CohenKuhi1979};  }
\tablenotetext{~}{4:  \citet{Herczeg2008};  5:  \citet{White2001}; 6:  \citet{Kenyon1995};  }
\tablenotetext{~}{7:  \citet{Gullbring1998}; 8:  \citet{Nguyen2009};  9:  \citet{Valenti1993};}
\tablenotetext{~}{10:  \citet{Gullbring2000}; 11:  \citet{Calvet2004};  12:  \citet{GarciaLopez2010};}
\tablenotetext{~}{13:  \citet{Santos2005};  14:  \citet{Mamajek2005}; 15:  \citet{Webb1999};}
\tablenotetext{~}{16:  \citet{Valenti2005};  17:  \citet{Herczeg2009}; 18: \citet{Sterzik1999};}
\tablenotetext{~}{19:  \citet{Ducourant2007}; 20:  \citet{Zuckerman2001};  21:  \citet{Mamajek2002};}
\tablenotetext{~}{22:  \citet{Herczeg2005}; 23: \citet{dezeeuw1999};  24:  \citet{Walter1994};}
\tablenotetext{~}{25:  \citet{Preibisch1999};  26:  \citet{Pascucci2007}; 27:  \citet{Bouvier1990};}
\tablenotetext{~}{28:  \citet{Hughes1994};  29:  \citet{Loinard2008}; 30:  \citet{Donati2007};}
\tablenotetext{~}{31: \citet{Basri1990}; 32:  \citet{Neuhauser2008}. }
\end{deluxetable}


